Gaussian Rough Paths Lifts via Complementary Young Regularity

Inspired by recent advances in singular SPDE theory, we use the Poincar\'e inequality on Wiener space to show that controlled complementary Young regularity is sufficient to obtain Gaussian rough paths lifts. This allows us to completely bypass assumptions on the 2D variation regularity of the covariance and, as a consequence, we obtain cleaner proofs of approximation statements (with optimal convergence rates) and show the convergence of random Fourier series in rough paths metrics under minimal assumptions on the coefficients (which are sharper than those in the existent literature).

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage[nottoc]{tocbibind}
\usepackage{graphicx}
\usepackage{amsmath,amsfonts,amsthm}
\usepackage{amssymb}
\usepackage{multirow,array}
\usepackage{comment}
\usepackage{enumitem}
%\usepackage{tkz-graph}
\usepackage[utf8]{inputenc}  
\usepackage[T1]{fontenc}
\usepackage{emptypage}
\usepackage{hyperref}
\usepackage{color}
\usepackage{mathrsfs}
\usepackage{tikz-cd}

\DeclareMathAlphabet{\mcb}{U}{BOONDOX-calo}{m}{n}
\SetMathAlphabet{\mcb}{bold}{U}{BOONDOX-calo}{b}{n}

%For backend=biber, use Bib(la)tex option: biber --input_directory="C:/Users/Ilya Chevyrev/Dropbox/Oxford/Own Notes/Common" %

% For backend=bibtex, use Bib(la)tex option: bibtex --include-directory="C:/Users/Ilya Chevyrev/Dropbox/Oxford/Own Notes/Common" %.aux

\usepackage[url=true,
doi=false,
maxbibnames=99,
isbn=false,
style=alphabetic,
backend=biber,
natbib=true,
sorting=nty]{biblatex}
\renewbibmacro{in:}{}
\bibliography{AllRefs}

%\numberwithin{equation}{section}
%\numberwithin{figure}{section}
%\newcounter{dummy}
%\numberwithin{dummy}{section}

\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
%\newenvironment{proof}[1][Proof]{\noindent\textbf{#1.} }{\ \rule{0.5em}{0.5em}}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}



\newcommand{\Nr}{\textnormal{Nr}}
\newcommand{\Vol}{\textnormal{Vol}}
\newcommand{\Tr}{\textnormal{Tr}}
\newcommand{\Cl}{\textnormal{Cl}}
\newcommand{\Hom}{\textnormal{Hom}}
\newcommand{\End}{\textnormal{End}}
\newcommand{\Ker}{\textnormal{Ker}}
\newcommand{\Aut}{\textnormal{Aut}}
\newcommand{\Sh}{\textnormal{Shuffle}}
\newcommand{\Id}{\textnormal{Id}}
\newcommand{\diam}{\textnormal{diam}}
\newcommand{\Diag}{\textnormal{Diag}}
\newcommand{\ExpSig}{\textnormal{ESig}}
\newcommand{\supp}{\textnormal{supp}}
\newcommand{\Lip}{\textnormal{Lip}}
\newcommand{\sign}{\textnormal{sign}}
\newcommand{\loc}{\textnormal{loc}}
\newcommand{\Lie}{\textnormal{Lie}}
\newcommand{\Vect}{\textnormal{Vect}}
\newcommand{\diver}{\textnormal{div}}
\newcommand{\reg}{\textnormal{reg}}
\newcommand{\ex}{\textnormal{ex}}
\newcommand{\ad}{\textnormal{ad}}
\newcommand{\Ad}{\textnormal{Ad}}
\newcommand{\grad}{\textnormal{grad}}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\mcK}{\mathcal{K}}
\newcommand{\SSS}{\mathcal{S}}
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\Zcal}{\mathcal{Z}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcE}{\mathcal{E}}

\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\Q}{\mathbb Q}
\newcommand{\F}{\mathbb F}
\newcommand{\K}{\mathbb K}
\newcommand{\T}{\mathbb T}
\newcommand{\bbA}{\mathbb{A}}

\newcommand{\X}{\mathbf X}
\newcommand{\x}{\mathbf x}
\newcommand{\y}{\mathbf y}
\newcommand{\z}{\mathbf z}
\newcommand{\bfn}{\mathbf n}
\newcommand{\w}{\mathbf w}
\newcommand{\mm}{\mathbf m}
\newcommand{\hh}{\mathbf h}
\newcommand{\B}{\mathbf B}
\newcommand{\ZZ}{\mathbf Z}
\newcommand{\bfPi}{\mathbf{\Pi}}
\newcommand{\Y}{\mcb{X}}

\newcommand{\var}[1]{#1\textnormal{-var}}
\newcommand{\Hol}[1]{#1\textnormal{-H{\"o}l}}
\newcommand{\gr}[1]{#1\textnormal{-gr}}\newcommand{\tri}[1]{#1\textnormal{-tri}}
\newcommand{\curv}[1]{#1\textnormal{-curv}}


\newcommand{\pvar}{p\textnormal{-var}}
\newcommand{\pprimevar}{p'\textnormal{-var}}
\newcommand{\qvar}{q\textnormal{-var}}
\newcommand{\onevar}{1\textnormal{-var}}
\newcommand{\twovar}{2\textnormal{-var}}
\newcommand{\rhovar}{\rho\textnormal{-var}}
\newcommand{\aHol}{\alpha\textnormal{-H{\"o}l}}
\newcommand{\pHol}{1/p\textnormal{-H{\"o}l}}
\newcommand{\pprimeHol}{1/p'\textnormal{-H{\"o}l}}
\newcommand{\qHol}{1/q\textnormal{-H{\"o}l}}
\newcommand{\betaHol}{\beta\textnormal{-H{\"o}l}}
\newcommand{\aprimeHol}{\alpha'\textnormal{-H{\"o}l}}
\newcommand{\oneHol}{1\textnormal{-H{\"o}l}}

\newcommand{\EEE}[1]{\mathbb E \left[ #1 \right]}
\newcommand{\EEEover}[2]{\mathbb E^{#1} \left[ #2 \right]}
\newcommand{\PPPover}[2]{\mathbb P^{#1} \left[ #2 \right]}
\newcommand{\EEEunder}[2]{\mathbb E_{#1} \left[ #2 \right]}
\newcommand{\Var}[1]{\textnormal{Var} \left[ #1 \right]}
\newcommand{\Diff}{\textnormal{Diff}}
\newcommand{\Homeo}{\textnormal{Homeo}}
\newcommand{\PPP}[1]{\mathbb{P} \left[ #1 \right]}
\newcommand{\QQQ}[1]{\Q \left[ #1 \right]}
\newcommand{\cv}[1]{\textnormal{cv}\left( #1 \right)}
\newcommand{\ob}[1]{\textnormal{ob}\left( #1 \right)}
\newcommand{\spn}[1]{\textnormal{span}\left( #1 \right)}
\newcommand{\id}{\textnormal{id}}
\newcommand{\norm}[1]{\left|\left|#1 \right|\right|}
\newcommand{\normt}[1]{\left|\left|\left|#1 \right|\right|\right|}
\newcommand{\norms}[1]{\left|#1 \right|}
\newcommand{\normc}{\norm{\cdot}}
\newcommand{\normtc}{\normt{\cdot}}
\newcommand{\1}[1]{\mathbf 1 \{#1\}}
\newcommand{\0}{\mathbf 0}
\newcommand{\LLL}{\mathbf L}
\newcommand{\GL}{\mathbf{GL}}
\newcommand{\LMC}{\mathbf{LMC}}
\newcommand{\Lyons}{S}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bfOmega}{\mathbf{\Omega}}
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\SC}{\mathscr{C}}

\newcommand{\mfu}{\mathfrak u}
\newcommand{\mfg}{\mathfrak g}
\newcommand{\mfG}{\mathfrak G}
\newcommand{\llie}{\mathfrak l}
\newcommand{\h}{\mathfrak h}
\newcommand{\gl}{\mathfrak {gl}}
\newcommand{\su}{\mathfrak{su}}
\newcommand{\symp}{\mathfrak{sp}}
\newcommand{\m}{\mathfrak m}
\newcommand{\s}{\mathfrak s}
\newcommand{\mfL}{\mathfrak L}
\newcommand{\mft}{\mathfrak t}
\newcommand{\Tfrak}{\mathfrak T}
\newcommand{\nfrak}{\mathfrak n}
\newcommand{\ofrak}{\mathfrak o}
\newcommand{\efrak}{\mathfrak e}
\newcommand{\Ffrak}{\mathfrak F}
\newcommand{\Ufrak}{\mathfrak U}
\newcommand{\Mfrak}{\mathfrak M}
\newcommand{\mfK}{\mathfrak K}
\newcommand{\mfI}{\mathfrak I}
\newcommand{\mfl}{\mathfrak l}

\newcommand{\DD}{\mathscr{D}}
\newcommand{\BB}{\mathscr{B}}
\newcommand{\eps}{{\varepsilon}}


\newcommand{\gen}[1]{\langle #1 \rangle}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\roof}[1]{\lceil #1 \rceil}
\newcommand{\scal}[1]{\langle #1 \rangle}
\newcommand{\mrd}{\mathop{}\!\mathrm{d}}

\newcommand{\midset}{\,\middle|\,}

\newcommand\restr[2]{{\left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

\def\eqd{\,{\buildrel \mcD \over =}\,}
\def\neqd{\,{\buildrel \mcD \over \neq}\,}
\def\convd{\,{\buildrel \mcD \over \rightarrow}\,}

\makeatother

\usepackage[english]{babel}

\def\ds{\displaystyle}
\def\oa#1{\overrightarrow{#1}}
\def\row#1#2{{#1}_1,\,\ldots,{#1}_{#2}}
\def\brow#1#2{{\bf {#1}}_1,\,\ldots,{\bf {#1}}_{#2}}
\def\lcomb#1#2#3{{#1}_1{#2}_1+{#1}_2{#2}_2+\cdots +{#1}_{#3}{#2}_{#3}}
\def\blcomb#1#2#3{{#1}_1{\bf {#2}}_1+{#1}_2{\bf {#2}}_2+\cdots 
+{#1}_{#3}{\bf {#2}}_{#3}}
\def\lcm#1#2{{\rm lcm}\>(#1,#2)}

\newcommand{\hol}{\textnormal{hol}}
\newcommand{\mbi}{\mathbf{i}}
